Is Bellman Equation Enough for Learning Control?

The Bellman equation and its continuous-time counterpart, the Hamilton-Jacobi-Bellman (HJB) equation, serve as necessary conditions for optimality in reinforcement learning and optimal control. While the value function is known to be the unique solution to the Bellman equation in tabular settings, we demonstrate that this uniqueness fails to hold in continuous state spaces. Specifically, for linear dynamical systems, we prove the Bellman equation admits at least $\binom{2n}{n}$ solutions, where $n$ is the state dimension. Crucially, only one of these solutions yields both an optimal policy and a stable closed-loop system. We then demonstrate a common failure mode in value-based methods: convergence to unstable solutions due to the exponential imbalance between admissible and inadmissible solutions. Finally, we introduce a positive-definite neural architecture that guarantees convergence to the stable solution by construction to address this issue.

==> sections/contribution.tex <==
\contribution{
    % Contribution
    We prove that solutions to the Bellman equation in continuous state and action spaces are generally non-unique, even under standard assumptions (e.g., smooth dynamics, discount factors). Furthermore, we demonstrate that value-based learning approaches frequently converge to unstable solutions, directly linking this non-uniqueness to practical failures in closed-loop control.
    }
    {
    While prior work established uniqueness in finite settings~\citep{bellman1957dynamic, blackwell1965discounted, sutton1988learning} and identified edge cases of non-uniqueness in continuous spaces (e.g., undiscounted or nonsmooth problems)~\citep{misztela2018nonuniqueness, HOSOYA2024102940, xuan2024uniqueness}, our results show non-uniqueness persists generically—exposing a broader, underappreciated limitation of value-based reinforcement learning.
    }

\contribution{
    % Contribution
    For linear dynamical systems, we derive an exact lower bound of $\binom{2n}{n}$ distinct solutions to the Bellman equation, yet only \emph{one} corresponds to a stable controller. This exponential imbalance explains why learning methods struggle to identify viable policies in high dimensions--a phenomenon we term the \emph{curse of dimensionality in solution space}, mirroring the computational curse of dimensionality in tabular settings. }
    {
    % Caveat:
    Though inspired by the solution to algebraic Riccati equation \citep{willems1971least, lancaster1995algebraic}, we provide novel linear-algebraic proofs (avoiding functional analysis) and explicitly characterize how discount factors affect the results.
    }
\contribution{
    % Contribution
    We introduce the use of positive-definite neural architectures to exclude unstable solutions from being learned and demonstrate their effectiveness in solving \emph{nonlinear} control problems.
    }
    {
    % Caveat:
    The key insight behind the use of positive-definite models is the close relationship between the value function and Lyapunov function. This opens up a new possibility to connect the value-based approach with the safe reinforcement learning community~\citep{brunke2022safe, dawson2022safe, dawson2023safe}. 
    }

==> sections/summary.tex <==
\summary{
The Bellman equation and its continuous-time counterpart, the Hamilton-Jacobi-Bellman (HJB) equation, serve as necessary conditions for optimality in reinforcement learning and optimal control. 
While the value function is known to be the unique solution to the Bellman equation in tabular settings, we demonstrate that this uniqueness \textbf{fails to hold} in continuous state spaces. 
Specifically, for linear dynamical systems, we prove the Bellman equation admits at least $\binom{2n}{n}$ solutions, where $n$ is the state dimension. 
Crucially, \textbf{only one} of these solutions yields both an optimal policy and a stable closed-loop system. 
We then demonstrate a common failure mode in value-based methods: convergence to unstable solutions due to the exponential imbalance between stable and unstable solutions. 
Finally, we introduce a positive-definite neural architecture that guarantees convergence to the stable solution by construction to address this issue.
}
